Modeling Exemplification in Long-form Question Answering via Retrieval

Exemplification is a process by which writers explain or clarify a concept by providing an example. While common in all forms of writing, exemplification is particularly useful in the task of long-form question answering (LFQA), where a complicated answer can be made more understandable through simple examples. In this paper, we provide the first computational study of exemplification in QA, performing a fine-grained annotation of different types of examples (e.g., hypotheticals, anecdotes) in three corpora. We show that not only do state-of-the-art LFQA models struggle to generate relevant examples, but also that standard evaluation metrics such as ROUGE are insufficient to judge exemplification quality. We propose to treat exemplification as a \emph{retrieval} problem in which a partially-written answer is used to query a large set of human-written examples extracted from a corpus. Our approach allows a reliable ranking-type automatic metrics that correlates well with human evaluation. A human evaluation shows that our model's retrieved examples are more relevant than examples generated from a state-of-the-art LFQA model.

==> figures/_example_personal_info.tex <==
\begin{figure}
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.347058823529412,0.458823529411765,0.641176470588235}
\definecolor{color1}{rgb}{0.798529411764706,0.536764705882353,0.389705882352941}

\begin{axis}[
font=\small,
axis line style={white!80!black},
legend cell align={left},
legend style={fill opacity=0.8, 
draw opacity=1, text opacity=1, at={(0.1, 1)}, draw=white!80!black, font=\tiny},
height=.3\textwidth,
width=.43\textwidth,
tick align=outside,
unbounded coords=jump,
x grid style={white!80!black},
% xlabel=\textcolor{white!15!black}{dataset},
%xmajorticks=false,
xmin=-0.5, xmax=2.5,
xtick style={color=white},
xtick={0,1,2},
xticklabels={Books3,ELI5,NQ},
y grid style={white!80!black},
ylabel=\textcolor{white!15!black}{\% Example},
y label style={at={(axis description cs:.2,.4)},anchor=south, font=\small},
% ymajorgrids,
ymajorticks=false,
ymin=0, ymax=113,
ytick style={color=white!15!black}
]



% 2 
\draw[draw=white,fill=color1] (axis cs:-0.4,0) rectangle (axis cs:0,2.35294117647059);
% 97
\draw[draw=white,fill=color0] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,97.6470588235294);
% 11 
\draw[draw=white,fill=color1] (axis cs:0.6,0) rectangle (axis cs:1,11.4942528735632);
% 88 
\draw[draw=white,fill=color0] (axis cs:1,0) rectangle (axis cs:1.4,88.5057471264368);
% 1 
\draw[draw=white,fill=color1] (axis cs:1.6,0) rectangle (axis cs:2,1.12359550561798);
% 98
\draw[draw=white,fill=color0] (axis cs:2,0) rectangle (axis cs:2.4,98.876404494382);

\addlegendimage{ybar,ybar legend,draw=white,fill=color1}
\addlegendentry{Personal}
\addlegendimage{ybar,ybar legend,draw=white,fill=color0}
\addlegendentry{Non-personal}


\addplot [line width=1.08pt, white!26!black, forget plot]
table {%
-0.2 nan
-0.2 nan
};
\addplot [line width=1.08pt, white!26!black, forget plot]
table {%
0.8 nan
0.8 nan
};
\addplot [line width=1.08pt, white!26!black, forget plot]
table {%
1.8 nan
1.8 nan
};
\addplot [line width=1.08pt, white!26!black, forget plot]
table {%
0.2 nan
0.2 nan
};
\addplot [line width=1.08pt, white!26!black, forget plot]
table {%
1.2 nan
1.2 nan
};
\addplot [line width=1.08pt, white!26!black, forget plot]
table {%
2.2 nan
2.2 nan
};
\draw (axis cs:-0.2,2.35294117647059) node[
  scale=0.9,
  anchor=south,
  text=black,
  rotate=0.0
]{2};
\draw (axis cs:0.2,97.6470588235294) node[
  scale=0.9,
  anchor=south,
  text=black,
  rotate=0.0
]{98};
\draw (axis cs:0.8,11.4942528735632) node[
  scale=0.9,
  anchor=south,
  text=black,
  rotate=0.0
]{11};
\draw (axis cs:1.2,88.5057471264368) node[
  scale=0.9,
  anchor=south,
  text=black,
  rotate=0.0
]{89};
\draw (axis cs:1.8,1.12359550561798) node[
  scale=0.9,
  anchor=south,
  text=black,
  rotate=0.0
]{1};
\draw (axis cs:2.2,98.876404494382) node[
  scale=0.9,
  anchor=south,
  text=black,
  rotate=0.0
]{99};
\end{axis}

\end{tikzpicture}
\caption{Distribution of examples with personal information.}
\label{fig:personal_info}
\end{figure}


==> figures/_example_real_hypothetical.tex <==
% This file was created with tikzplotlib v0.9.15.
\begin{figure}
\begin{tikzpicture}

\definecolor{color1}{rgb}{0.347058823529412,0.458823529411765,0.641176470588235}
\definecolor{color0}{rgb}{0.798529411764706,0.536764705882353,0.389705882352941}

\begin{axis}[
font=\small,
axis line style={white!80!black},
legend cell align={left},
legend style={fill opacity=0.8, 
draw opacity=1, text opacity=1, at={(0.1, 1)}, draw=white!80!black, font=\tiny},
height=.3\textwidth,
width=.43\textwidth,
tick align=outside,
unbounded coords=jump,
x grid style={white!80!black},
% xlabel=\textcolor{white!15!black}{dataset},
%xmajorticks=false,
xmin=-0.5, xmax=2.5,
xtick style={color=white},
xtick={0,1,2},
xticklabel style={font=\small, color=black},
xticklabels={Books3,ELI5,NQ},
y grid style={white!80!black},
ylabel=\textcolor{white!15!black}{\% Example},
y label style={at={(axis description cs:.2,.4)},anchor=south, font=\small},
% ymajorgrids,
ymajorticks=false,
ymin=0, ymax=100,
ytick style={color=white!15!black}
]
\draw[draw=white,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0,11.7647058823529);
\addlegendimage{ybar,ybar legend,draw=white,fill=color0}
\addlegendentry{hypothetical}

\draw[draw=white,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1,32.183908045977);
\draw[draw=white,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2,15.7303370786517);
\draw[draw=white,fill=color1] (axis cs:-2.77555756156289e-17,0) rectangle (axis cs:0.4,88.2352941176471);
\addlegendimage{ybar,ybar legend,draw=white,fill=color1}
\addlegendentry{real}

\draw[draw=white,fill=color1] (axis cs:1,0) rectangle (axis cs:1.4,67.816091954023);
\draw[draw=white,fill=color1] (axis cs:2,0) rectangle (axis cs:2.4,84.2696629213483);
\addplot [line width=1.08pt, white!26!black, forget plot]
table {%
-0.2 nan
-0.2 nan
};
\addplot [line width=1.08pt, white!26!black, forget plot]
table {%
0.8 nan
0.8 nan
};
\addplot [line width=1.08pt, white!26!black, forget plot]
table {%
1.8 nan
1.8 nan
};
\addplot [line width=1.08pt, white!26!black, forget plot]
table {%
0.2 nan
0.2 nan
};
\addplot [line width=1.08pt, white!26!black, forget plot]
table {%
1.2 nan
1.2 nan
};
\addplot [line width=1.08pt, white!26!black, forget plot]
table {%
2.2 nan
2.2 nan
};
\draw (axis cs:-0.2,11.7647058823529) node[
  scale=0.9,
  anchor=south,
  text=black,
  rotate=0.0
]{11};
\draw (axis cs:0.8,32.183908045977) node[
  scale=0.9,
  anchor=south,
  text=black,
  rotate=0.0
]{32};
\draw (axis cs:1.8,15.7303370786517) node[
  scale=0.9,
  anchor=south,
  text=black,
  rotate=0.0
]{15};
\draw (axis cs:0.2,88.2352941176471) node[
  scale=0.9,
  anchor=south,
  text=black,
  rotate=0.0
]{88};
\draw (axis cs:1.2,67.816091954023) node[
  scale=0.9,
  anchor=south,
  text=black,
  rotate=0.0
]{67};
\draw (axis cs:2.2,84.2696629213483) node[
  scale=0.9,
  anchor=south,
  text=black,
  rotate=0.0
]{84};
\end{axis}

\end{tikzpicture}
\caption{Distribution of real/hypothetical examples.}
\label{fig:real_hypothetical}
\end{figure}


==> sections/analysis.tex <==
\section{Analysis}
\label{sec:analysis}



% \swcomment{
% \begin{itemize}
%     \item error analysis (Do models tend to make mistakes for certain categories?)
% \end{itemize}
% }

==> tables/generated_example_analysis.tex <==

\begin{table*}[t!]
\small
%\begin{tabular}{ m{3.4cm}  m{3.4cm}} 

\begin{center}
% \begin{adjustbox}{max width=1\textwidth}

\begin{tabular}{m{1.5cm}m{1cm}m{5cm}m{5cm}}  
 \toprule
 \textbf{Type} & \textbf{Personal} & \textbf{Left context} & \textbf{Generated Example} \\ 
  % \midrule
  % \textbf{Real example from NQ} & \\
  \midrule
  Hypothetical &&  \textbf{Question:}  What would happen if the US govt cut all foreign aid?
  \textbf{Answer:} [...]4 billion - Economic and Military aid for Pakistan, Egypt, and Jordan. The goal is to have a few people in the mideast who call us allies. Essentially, we buy their cooperation. \textbf{That cooperation is sometimes useful.} & For example, \textit{For everyone here talking about how a lot of aid works: If we put money towards helping foreign countries rebuild, we are imposing restrictions on domestic activity. Our governments don't want people to domesticate animals domestically; they want people to be able to make their own own food and farm/milk and so on. Other countries don't like that, so they are trying to prevent people from doing that. } \\
  % & 
  % analysis 
  % Hypothetical example \\ 
  \midrule
  Real && \textbf{Question:}  Why are there so few venomous creatures in the UK and Northern Europe? \textbf{Answer: } [...] Since there are fewer species further north (because there are fewer resources like sunlight), this results in fewer overall numbers of venomous/toxic species. \textbf{I would argue, however, that there is still a similar percentage of *toxic* species, compared to the tropics.} & For example, \textit{smaller number of poisonous species in the UK because they have the traditional authority; and B) that a lot of poisonous species are actually useful to us. In my opinion, both are not true (as far as I am aware) and both are moot in the absence of culture or government control of species.} \\ 
  % & 
  % analysis 
  % The model generated a real example (UK). \\ 
  \midrule 
  Real & \checkmark & \textbf{Question:} How do hundreds of animators work together on the same project file when making a big budget animated movie? \textbf{Answer:} You don't usually work on the same files because everything is split up between the departments. \textbf{I haven't used USD yet but I have encountered the following workflow in different studios (using Maya).} & 
  For example, \textit{As a starting point: I'm a post graduate and work in the final sector of the project, not the project itself. Most of the work is done with other studios around the world who are made up of multiple departments. What it really comes down to is that if you want to work on one project, you start with every sub-department and have a staff member do it for you. The sub-department is actually under no obligation to support the project at all, but will do whatever they can to deliver the project and if they don't get it done then it's a loss for them. } \\
  % & The model generated a personal anecdote style example. \\ 
  
 \bottomrule
 
\end{tabular}
% \end{adjustbox}

\end{center}
\caption{Analysis on generated examples. The model learned to generate different types of examples and yet most of them are (a) unrelated to the context (b) contains non-factual contents or contradictions.}
\label{tab:generated_example_analysis}

\end{table*}

==> tables/rouge_analysis.tex <==
\begin{table*}
\small
%\begin{tabular}{ m{3.4cm}  m{3.4cm}} 

\begin{center}
% \begin{adjustbox}{max width=1\textwidth}

\begin{tabular}{m{3.5cm}m{3.5cm}m{3.5cm}m{3.5cm}}  
 \toprule
 \textbf{Left context}  & \textbf{Ground-truth} & \textbf{Retrieved} & \textbf{Top ROUGE} \\ 
  % \midrule
  % \textbf{Real example from NQ} & \\
  \midrule
  % 4.0/0.107 &  
  % \textbf{Question:}  Why are Chinese and Japanese people called "Asians", but Indians aren't?
  % \textbf{Answer:} [...] 
%   Ethnically, Chinese, Koreans, etc. are all different but because they have similar physical characteristics they are often lumped into a single race. Using race as means of grouping people is troublesome because you can't account for mixed backgrounds. & For example, if you have one white and one black parent what does that make you racially?
%   & 
%   For example, an African-American and a Jamaican who are both dark-skinned would be lumped into the same race, but despite a similarity in skin color these ethnic groups are as different genetically as Africans and white Europeans. (\textbf{R}:0.107/\textbf{H}:4.0) & There are a number of other laws on the books that are similar - i.e., regulation of personal behavior that largely impacts the individual and perhaps only tangentially affect a larger group (drug prohibition, for example).(\textbf{R}:0.14)\\
  % & 
  % analysis 
  % Hypothetical example \\ 
  % \midrule
  % 4.5/0.123 & 
  % \textbf{Question:} What does the term "identity politics" mean? \textbf{Answer: }
%   Identity politics is the tendency to view all political issues in terms of how those issues affect a particular group, most often a race, gender, religion, or sexual orientation.& For example, when Melania Trump was accused of plagiarizing Michelle Obama's convention speech, some people accused Melania of racism because Melinia is a white woman stealing (or ""appropriating"") from a black woman. & For example, if a politician said, "You should vote for me because I'm  < race / gender / religion / sexual orientation > ," or "I'm appointing this person because they're  < race / gender / religion / ethnicity > ." (\textbf{R}:0.123/\textbf{H}:4.5) & In the UK there is the criminal offence *Leaving a Vehicle in a Dangerous Position* , for example on a blind corner. (\textbf{R}:0.20)\\ 
%   \midrule
  evolution is not a force towards the optimum, it's a force towards the minimum necessary. & for example, if grass was poisonous, it would be better for its survival, as less animals would come eat it.  & For example, we move incredible slowly when compared to the maximum speed allowed in the universe. (\textbf{R}:0.111/\textbf{H}:5.0) & For example, if a certain percentage of snakes are venomous, then the more snakes in a given area the more venomous. (\textbf{R}:0.22) \\
  % 5.0/0.169 & 
  % \textbf{Question:} Why does 100\% humidity not mean water everywhere? \textbf{Answer:} 
%   Humidity is the percent of water in the air. The reason that 100\% humidity would not mean water everywhere is due to the fact that the percentage you are referring to only suggests the amount of water the air can hold. & For example, when it's hot outside air expands meaning their is more room between air particles which means more water can fill into the gaps. & For example,if the current relative humidity is 65 percent, the air is holding 65 percent of the total amount of moisture that it is capable of holding at that temperature and pressure. (0.169/5.0) & \\ 
  
 \bottomrule
 
\end{tabular}
% \end{adjustbox}

\end{center}
\caption{Retrieved examples with high \textbf{H}uman rating and highest \textbf{R}OUGE-L w.r.t. ground truth.}
\label{tab:rouge_analysis}

\end{table*}
